Community Detection in Networks with Node Attributes

Community detection algorithms are fundamental tools that allow us to uncover organizational principles in networks. When detecting communities, there are two possible sources of information one can use: the network structure, and the features and attributes of nodes. Even though communities form around nodes that have common edges and common attributes, typically, algorithms have only focused on one of these two data modalities: community detection algorithms traditionally focus only on the network structure, while clustering algorithms mostly consider only node attributes. In this paper, we develop Communities from Edge Structure and Node Attributes (CESNA), an accurate and scalable algorithm for detecting overlapping communities in networks with node attributes. CESNA statistically models the interaction between the network structure and the node attributes, which leads to more accurate community detection as well as improved robustness in the presence of noise in the network structure. CESNA has a linear runtime in the network size and is able to process networks an order of magnitude larger than comparable approaches. Last, CESNA also helps with the interpretation of detected communities by finding relevant node attributes for each community.

==> 001summary.tex <==
\xhdr{Strength of our model}
\begin{itemize}
\item Model `A': We model direct relationship between community affiliation and node attributes.
\item Hard-membership: We allow nodes to belong to multiple communities simultaneously.
\item Scalability: We build on BigCLAM that is the most scalable method. We lose to BigCLAM only by a constant factor (30\%).
\end{itemize}



==> 010intro_short.tex <==
\parttitle{State the problem: community detection}
One of the most important tasks in understanding networks is that of identifying sets of related nodes, or \emph{network communities}. Fundamentally, communities allow us to discover high-level structure among interacting objects. For example, in a social network, such high-level structures might be groups of friends who attended the same school, or who come from the same hometown~\cite{julian12circles}; in a protein interaction network, high-level structures might be functional modules of interacting proteins that share some common role~\cite{Ahn10LinkCommunitiesNature}; in a co-authorship network, high-level structures might be scientific communities~\cite{palla05_OveralpNature}. Identifying these structures allows us to identify users (or proteins etc.) that are similar to each other, to infer missing attributes, or to predict which connections are likely to form in the future.

\parttitle{How can we solve the problem? Node clustering, we can do on networks or attributes, or both!}
Identifying such communities in a given network, \ie, community detection, is essentially clustering the nodes in the networks.
There are two sources of data that we can use for node clustering: the connectivity structure of the nodes and the attributes of the nodes.
The underlying intuition is that the nodes in the same communities are more likely to be connected to each other~\cite{jaewon11agmmodel2}, and to have similar attributes each other~\cite{Crandall08Selection,julian12circles}.
For example, proteins belonging to the same complex are more likely to interact each other and to possess the same chemical properties~\cite{Ahn10LinkCommunitiesNature}; individuals in a particular research community would collaborate more often and share research interests~\cite{palla05_OveralpNature}.
Ideally, we should consider both sources of information together because, if one source of information is missing or noisy, the other can make up for it.


\parttitle{Why is it hard? Communities overlap}
Considering both node attributes and network topology for community detection is challenging as one has to combine two very different modalities of information.
Moreover, the fact that communities overlap with each other~\cite{Ahn10LinkCommunitiesNature, palla05_OveralpNature,jaewon13agmfast} brings another huge challenge,
\ie, we need to allow nodes to belong to multiple communities (multi-assignment clustering).
There are many existing methods that combine the network and node attribute for single-assignment clustering~\cite{Ester06Cluster,Ruan13CODICIL,Zhou09Clustering}; however, their applicability is limited as they cannot detect overlapping communities.

\begin{table}[t]
\small
\begin{center}
\begin{tabular}{p{0.2\textwidth}|c|c|c|c}
\hline
Method & \pbox{0.07\textwidth}{$O$} & \pbox{0.07\textwidth}{$H$} & \pbox{0.09\textwidth}{$D$} & \pbox{0.09\textwidth}{$N$} \\ \hline
 \pbox{0.2\textwidth}{\cite{Cohen11BlockLDA,LinkLDA,RelationalLDA, Sun12AttributeCluster, Xu12AttributedGraph}} & \cmark & \xmark & \cmark & 85,000 \\ \hline
 \pbox{0.2\textwidth}{\cite{Ester06Cluster,Ruan13CODICIL,Zhou09Clustering}} & \xmark & \cmark & \xmark &  100,000\\ \hline
% Moser et al.~\cite{Moser09Cluster} & \cmark  & \cmark &  & 3k\\ \hline
% Yang et al.~\cite{Zhou09Clustering} &  & \cmark &  & 5k\\ \hline
 \pbox{0.2\textwidth}{\cite{julian12circles}}& \cmark& \cmark & \xmark & 5,000 \\ \hline
 \textbf{Our model} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{1,000,000}\\
\hline
\end{tabular}
\end{center}
  \caption{Summary of the existing methods. $O$: Detecting overlapping communities?, $H$: Detecting hard-membership? $D$: Communities generating node attributes? (Fig.~\ref{fig:model.A}). $N$: the number of nodes that the method can process within 10 hours. Refer to Sec.~\ref{sec:related} for details.
  }
  \label{tab:baselines}
  \vspace{-8mm}
\end{table}


\parttitle{Why previous methods do not work? soft membership, independence}
Recently, a few approaches have been developed to detect overlapping communities based on both sources of information~\cite{Cohen11BlockLDA,julian12circles} (Table~\ref{tab:baselines}).
Many such methods \cite{Cohen11BlockLDA,LinkLDA, Sun12AttributeCluster,Xu12AttributedGraph} are based on topic models and thus assumes ``soft-membership'', \ie, a node's membership is modeled in terms of its probability of belonging to a community.
Whereas soft-membership is a natural way to represent topic memberships of a document, it is not appropriate for modeling community memberships because it does not allow a node to have high membership strength to multiple communities {\em simultaneously}.
%
On the other hand, \cite{julian12circles} developed an overlapping community detection method based on ``hard-membership'', which can assign a node to multiple communities simultaneously.
However, the method did not correctly capture the interplay between communities, node attributes, and the underlying network
because the method assumes that the node attributes are given {\em independently} from communities to generate networks (Fig.~\ref{fig:model.V}).
This assumption on independence goes against our intuition that communities influence both the network structure and node attributes (Fig.~\ref{fig:model.A}).
Our experimental results also suggest that modeling the dependency between the node attributes and communities leads to better performance.
%
Finally, all existing methods are unable to handle large-scale networks: the networks analyzed typically consist of at most a few thousand nodes~\cite{julian12circles}.
We discuss related work in more details in Sec.~\ref{sec:related}.
\begin{figure}[t]
\centering
  \subfigure[]{\label{fig:model.A}\includegraphics[height=0.09\textwidth]{diagram_A.eps}}
  \hspace{5mm}
  \subfigure[]{\label{fig:model.V}\includegraphics[height=0.09\textwidth]{diagram_V.eps}}
   \vspace{-2mm}
   \caption{
   Two ways of building models between a graph $G$, attributes $X$, and community membership $F$. Circles represent latent variables and squares represent manifest (observed) variables.
   }
   \label{fig:models}
   \vspace{-3mm}
\end{figure}



\xhdr{Present work: Efficient and accurate community detection in networks with node attributes}
The goal of this paper is to develop a high performance (accurate and scalable) community detection method for networks where node attributes are also available.
To do this, we present \fullmodel (\model), a novel scalable method that is based on a generative model for networks with node attributes.
Our model advances the existing models by making the modeling choices that lead to better performance; Our model employs hard-membership rather than soft-membership, and it assumes that the node attributes are generated from communities. To the best our knowledge, \model is the first method that models both hard-membership and the communities-attributes dependency.
To maximize scalability, our model builds on BigCLAM~\cite{jaewon13agmfast}, which is the state-of-the-art community detection method both in terms of accuracy and scalability.
Our method possesses all the strengths of BigCLAM: it can detect overlapping, non-overlapping, as well as hierarchically nested communities in large-scale networks.
While BigCLAM is solely based on the graph structure, however, our method considers \emph{both} node attributes and graph structure, which leads to better performance.

We build a probabilistic generative model where we assign a non-negative membership factor between each node and each community.
Our model then assumes that these membership factors generate both the edges between the nodes and the node attributes.
To generate the network edges, we employ the generative process from BigCLAM and other affiliation network models~\cite{breiger74groups,feld86focused}, where the observed edges arise due to shared community affiliations between pairs of nodes.
To generate the node attributes, we consider a set of logistic models so that members of each community tend to share common traits.


%
To identify communities from a given network with node attributes, we fit \model to the network and the attributes simultaneously, by identifying the most likely community memberships.
We develop a scalable, efficient fitting method based on block-coordinate ascent where we can update all model parameters in \emph{linear} time in the number of edges.



==> 020related_short.tex <==
In this section, we discuss the existing methods for community detection in networks with node attributes.
Our discussion focuses on two criteria, First, we consider how the methods jointly model communities, node attributes, and the underlying graph (network). Figure~\ref{fig:models} shows the two paradigms that are typically used.
On the left (Figure~\ref{fig:model.A}), community memberships $F$ generate both the graph $G$ and attributes $X$, while on the right (Figure~\ref{fig:model.V}) $F$ and $X$ are given independently and then the graph $G$ is generated by the interaction between $F$ and $X$.
Second, we focus on how the methods model the community memberships of individual nodes.
One way is to associate a probability with each node and community, \ie, each node has a ``soft membership'' to all communities.
The other way is to consider a binary variable for each node and community, \ie, ``hard membership''.
The methods based on hard membership can be further divided into two cases by whether the methods allow a node to belong to multiple communities (overlapping communities) or not (non-overlapping communities).


We first discuss single-assignment clustering methods for networks with node attributes~\cite{Ester06Cluster,Ruan13CODICIL,Zhou09Clustering}.
These methods construct a weighted graph based on an input graph and node attributes, and then run clustering algorithms on the weighted graph.
The clustering algorithms detect hard-membership because the output for each node is a membership to a single community.
However, these methods cannot detect overlapping communities.

Next, we discuss the methods that can detect overlapping communities.
We note that many existing methods~\cite{Cohen11BlockLDA,RelationalLDA,LinkLDA} are based on topic models~\cite{blei03lda}, which aim to find sets of documents that discuss the same topic based on word occurrences and links between documents.
%By representing nodes as documents and attributes as words, these models can be directly applied to the problems we investigate here.
These topic models are based on the paradigm in Figure~\ref{fig:model.A} where topic (community) memberships of documents (nodes) generate links (the graph) and words (attributes).
As for modeling community memberships, the topic models detect overlapping communities by finding soft-memberships (\ie, the probabilities stand for the fraction of words for topics).
We note that \cite{Sun12AttributeCluster, Xu12AttributedGraph} also belong to this type because these methods assume soft-membership and the paradigm in Fig.~\ref{fig:model.A}.
However, soft-membership is not the best way to model community memberships.
In soft membership, high membership strength from a node to one community by definition precludes high membership strength from the node to other communities.
This makes sense when nodes represent ``documents'' and communities represent ``topics'', since (for example), a document that discusses both \emph{politics} and \emph{sport} presumably does not discuss sport with the same strength as a document that discusses sport alone.
However, this assumption is no longer valid in other types of networks (\eg, in social networks), where nodes can have high membership strength to multiple communities simultaneously~\cite{julian12circles}.
Indeed, these topic models have been outperformed by methods that detect hard memberships~\cite{julian12circles,jaewon13agmfast}. Therefore, \model aims to detect hard memberships also.

Recently, \cite{julian12circles} developed a pseudo-boolean method that detects overlapping communities with hard-membership.
This model is based on the paradigm in Figure~\ref{fig:model.V}.
However, we note that the paradigm in Figure~\ref{fig:model.A} is a better paradigm than the paradigm in Figure~\ref{fig:model.V} due to the following key observation.
Conceptually, Fig.~\ref{fig:model.A} assumes a direct connection from $F$ to $X$; however, Figure~\ref{fig:model.V} assumes $F$ and $X$ are {\em marginally independent}.
This difference has a large practical advantage for Fig.~\ref{fig:model.A};
if $G$ is noisy (for example) Fig.~\ref{fig:model.A} still can infer $F$ from $X$. On the other hand, Fig.~\ref{fig:model.V} does not allow $F$ to be inferred from $X$.
Thus, we choose the paradigm in Fig.~\ref{fig:model.A} for our model.
%In our experiments (Sec.~\ref{sec:experiments}), we verify that \model achieves better accuracy than \cite{julian12circles}.% as the graph $G$ gets noisier.

Table~\ref{tab:baselines} summarizes our discussion for related work.
In summary, our model differs from all the existing method as we adopt hard-membership, overlapping communities, and the paradigm in Figure~\ref{fig:model.A}.
Our experiments \cite{jaewon13attributes} show that our design choices lead to improved performance.

